Single-Molecule-Sensitive FRET in Freely-Diffusing Attoliter Droplets

Fluorescence resonance energy transfer (FRET) from individual, dye-labeled RNA molecules confined in freely-diffusing attoliter-volume aqueous droplets is carefully compared to FRET from unconfined RNA in solution. The use of freely-diffusing droplets is a remarkably simple and high-throughput technique that facilitates a substantial increase in signal-to-noise for single-molecular-pair FRET measurements. We show that there can be dramatic differences between FRET in solution and in droplets, which we attribute primarily to an altered pH in the confining environment. We also demonstrate that a sufficient concentration of a non-ionic surfactant mitigates this effect and restores FRET to its neutral-pH solution value. At low surfactant levels, even accounting for pH, we observe differences between the distribution of FRET values in solution and in droplets which remain unexplained. Our results will facilitate the use of nanoemulsion droplets as attoliter volume reactors for use in biophysical and biochemical assays, and also in applications such as protein crystallization or nanoparticle synthesis, where careful attention to the pH of the confined phase is required.

==> table_Mixed_dates_10.tex <==
\begin{tabular}{|ll|llllllll|}
\hline
 $\mean{N_{th}}$ & Fig & $A$ & $\alpha$  &  $\beta$  &  $\mean{P}$ & $\sigma_d$ & $ \sigma_s$ & bins & $\mean{N_t}$  \\
\hline
  25 	&	 1a 	&	   0.80 	&	   19.63 	&	   11.61 	&	  0.628 	&	  0.094 	&	  0.083 	&	   1169 	&	    37.0 \\
  25 	&	 1a 	&	   0.20 	&	    6.32 	&	    2.49 	&	  0.718 	&	  0.149 	&	  0.078 	&	    303 	&	    37.7 \\
  75 	&	 1b 	&	   0.67 	&	   43.39 	&	   26.64 	&	  0.620 	&	  0.057 	&	  0.050 	&	    898 	&	    99.6 \\
  75 	&	 1b 	&	   0.33 	&	   13.04 	&	    6.64 	&	  0.663 	&	  0.106 	&	  0.048 	&	    472 	&	   100.5 \\
  75 	&	 1c 	&	   0.68 	&	   37.28 	&	   22.10 	&	  0.628 	&	  0.061 	&	  0.048 	&	    499 	&	   104.5 \\
  75 	&	 1c 	&	   0.32 	&	   14.20 	&	    6.05 	&	  0.701 	&	  0.108 	&	  0.046 	&	    241 	&	   104.5 \\
  50 	&	 1d 	&	   0.39 	&	   40.65 	&	   16.39 	&	  0.713 	&	  0.067 	&	  0.052 	&	   2055 	&	    85.1 \\
  50 	&	 1d 	&	   0.61 	&	    5.00 	&	    1.59 	&	  0.759 	&	  0.162 	&	  0.049 	&	   3369 	&	    87.0 \\
  60 	&	 1e 	&	   0.78 	&	   14.24 	&	    6.15 	&	  0.699 	&	  0.102 	&	  0.052 	&	    449 	&	    83.3 \\
  60 	&	 1e 	&	   0.22 	&	   22.67 	&	    4.00 	&	  0.850 	&	  0.067 	&	  0.040 	&	    126 	&	    83.8 \\
\hline
\end{tabular}
